Fragmentation, Price Formation, and Cross-Impact in Bitcoin Markets

In light of micro-scale inefficiencies induced by the high degree of fragmentation of the Bitcoin trading landscape, we utilize a granular data set comprised of orderbook and trades data from the most liquid Bitcoin markets, in order to understand the price formation process at sub-1 second time scales. To achieve this goal, we construct a set of features that encapsulate relevant microstructural information over short lookback windows. These features are subsequently leveraged first to generate a leader-lagger network that quantifies how markets impact one another, and then to train linear models capable of explaining between 10% and 37% of total variation in $500$ms future returns (depending on which market is the prediction target). The results are then compared with those of various PnL calculations that take trading realities, such as transaction costs, into account. The PnL calculations are based on natural $\textit{taker}$ strategies (meaning they employ market orders) that we associate to each model. Our findings emphasize the role of a market's fee regime in determining its propensity to being a leader or a lagger, as well as the profitability of our taker strategy. Taking our analysis further, we also derive a natural $\textit{maker}$ strategy (i.e., one that uses only passive limit orders), which, due to the difficulties associated with backtesting maker strategies, we test in a real-world live trading experiment, in which we turned over 1.5 million USD in notional volume. Lending additional confidence to our models, and by extension to the features they are based on, the results indicate a significant improvement over a naive benchmark strategy, which we also deploy in a live trading environment with real capital, for the sake of comparison.

==> preamble.tex <==

% \usepackage[utf8]{inputenc}


\usepackage{arxiv}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
%\usepackage{blindtext}
%\hypersetup{
  %   colorlinks=red,
  %  linkcolor=blue,
  %  filecolor=magenta,      
  %  urlcolor=cyan,
%}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage{graphicx}
% \usepackage{unicode-math}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{float}
\usepackage{epstopdf}




\usepackage{amsthm}

\usepackage[english]{babel}
\newtheorem{theorem}{Theorem}
% \theoremstyle{definition}
\newtheorem{definition}{Definition}[section]


\usepackage[colorlinks=true,linkcolor=blue,filecolor=green,citecolor=blue]{hyperref}

% \usepackage{setspace} 
% \usepackage[titles]{tocloft}
% \setlength{\cftbeforechapskip}{3pt}

%\usepackage{tocbasic}
%\DeclareTOCStyleEntry[
%  beforeskip=.2em plus 1pt,% default is 1em plus 1pt
%  pagenumberformat=\textbf
%]{tocline}{chapter}


\usepackage[utf8]{inputenc}
\usepackage{titletoc}
    \titlecontents{chapter}
    [0em] %
    {\medskip\bfseries}
    {\thecontentslabel\quad}%numbered chapters
    {}%numberless chapter
    {\hfill\contentspage}

    \titlecontents{section}[1.72em]{\smallskip}%
    {\thecontentslabel.\enspace}%numbered sections
    {}%numberless section
    {\titlerule*[1.2pc]{.}\contentspage}%
    

\usepackage[dvipsnames]{xcolor} 

%% In the below, create a macro for each one of you
% (just copy paste the two lines below, and replace every occurence of MC with you initials, update your name and choose your favorite colour)
\newcounter{noteMCctr} \setcounter{noteMCctr}{1}
\newcommand{\MC}[1]{\textbf{\textcolor{blue}{{{Mihai: \#\arabic{noteMCctr}: }}#1}} \addtocounter{noteMCctr}{1}}


\newcommand{\mc}[1]{\textcolor{blue}{#1}} 


    
\newcounter{noteZZctr} \setcounter{noteZZctr}{1}
\newcommand{\AS}[1]{\textbf{\textcolor{red}{{{Alex: \#\arabic{noteZZctr}: }}#1}} \addtocounter{noteZZctr}{1}}

\newcommand{\as}[1]{\textcolor{red}{#1}} 


\newcounter{noteXXctr} \setcounter{noteXXctr}{1}
\newcommand{\JA}[1]{\textbf{\textcolor{BurntOrange}{{{Jakob: \#\arabic{noteXXctr}: }}#1}} \addtocounter{noteXXctr}{1}}


% \newcommand{\as}[1]{\textcolor{BurntOrange}{#1}} 


\newcommand{\bb}{\hspace{-1mm} $\bullet$ }
% \usepackage[left=2 cm,right=2 cm,top=1.7 cm,bottom=1.7 cm,headsep=0.6 cm,footnotesep=0.6cm]{geometry}
    


\usepackage[%
    font={small,sf},
    labelfont=bf,
    format=hang,    
    format=plain,
    margin=0pt,
    width=0.8\textwidth,
]{caption}
% \usepackage{subfigure}    

\usepackage[list=true]{subcaption}

